Mono and Multi-objective Models for the Emergency Medical Service in the City of Belo Horizonte, Brazil

This work presents the facility location problem for maximum coverage in an emergency medical service called SAMU-BH, located in Belo Horizonte, Minas Gerais, Brazil. The purpose of the proposed model is to find the best locations for its ambulances in order to provide faster in-site assistance whenever necessary. First, it develops a mono-objective model to maximize the coverage rate, defined as the number of calls attended before a target time. Based on the Facility Location and Equipment Emplacement Technique (FLEET) model, a novel mathematical model is proposed, called FLEET-IC, which can work with independent coverages. Secondly, it proposes a multi-objective model to increase total coverage while reducing the number of installed bases. The results show that the mono-objective model's application increases the coverage rate up to 48%, considering the busy fraction factor and up to 26% without it. It also analyzes the effect on the coverage rate of the inclusion of additional ambulances.

==> txocupacao.tex <==
\begin{table}[!htb]
    \centering
    \caption{Taxa de Ocupação - USAs e USBs}
    \label{tab:txocupacaoA}
    \begin{tabular}{lrrrrrr}
        \toprule
\multicolumn{1}{c}{Mês de} & \multicolumn{2}{c}{USA - Tempos totais (em horas)} & \multicolumn{1}{c}{Fração} & \multicolumn{2}{c}{USB - Tempos totais (em horas)} & \multicolumn{1}{c}{Fração} \\

\multicolumn{1}{c}{Referência} & \multicolumn{1}{c}{Em Atendimento} & \multicolumn{1}{c}{Disponível} &  \multicolumn{1}{c}{$q_1$} & \multicolumn{1}{c}{Em Atendimento} & \multicolumn{1}{c}{Disponível} & \multicolumn{1}{c}{$q_2$} \\
        \midrule
Maio-2016	&	763,15	&	4464	&	0,17 \\
Junho-2016	&	806,42	&	4320	&	0,19 \\
Julho-2016	&	699,27	&	4464	&	0,16 \\
Agosto-2016	&	651,72	&	4464	&	0,15 \\
Setembro-2016	&	617,52	&	4320	&	0,14 \\
Outubro-2016	&	600,33	&	4464	&	0,13 \\
Novembro-2016	&	592,82	&	4320	&	0,14 \\
Dezembro-2016	&	691,82	&	4464	&	0,15 \\
Janeiro-2017	&	634,63	&	4464	&	0,14 \\
Fevereiro-2017	&	534,12	&	4032	&	0,13 \\
Março-2017	&	636,02	&	4464	&	0,14 \\
Abril-2017	&	618,80	&	4320	&	0,14 \\
        \midrule
Tempos Totais e média de $q$	&	7846,60	&	52560	&	0,15 \\
        \bottomrule
    \end{tabular}
    \fonte{Autora, 2018}
\end{table}

